Chart-HQA: A Benchmark for Hypothetical Question Answering in Charts

Multimodal Large Language Models (MLLMs) have garnered significant attention for their strong visual-semantic understanding. Most existing chart benchmarks evaluate MLLMs' ability to parse information from charts to answer questions. However, they overlook the inherent output biases of MLLMs, where models rely on their parametric memory to answer questions rather than genuinely understanding the chart content. To address this limitation, we introduce a novel Chart Hypothetical Question Answering (HQA) task, which imposes assumptions on the same question to compel models to engage in counterfactual reasoning based on the chart content. Furthermore, we introduce HAI, a human-AI interactive data synthesis approach that leverages the efficient text-editing capabilities of LLMs alongside human expert knowledge to generate diverse and high-quality HQA data at a low cost. Using HAI, we construct Chart-HQA, a challenging benchmark synthesized from publicly available data sources. Evaluation results on 18 MLLMs of varying model sizes reveal that current models face significant generalization challenges and exhibit imbalanced reasoning performance on the HQA task.

==> Sections/10_Analysis.tex <==
\begin{table}[t]
    \centering
    \caption{Ablations of {\model} on ChartQA and Chart-HQA.}
    \begin{tabular}{p{0.48\columnwidth}cc}
    \toprule
        Method & ChartQA & Chart-HQA  \\ 
    \midrule
        {\model} & \textbf{81.20} & \textbf{56.89} \\
    \midrule
         $w/o$ collaborative reward & 79.70 & 53.66 \\ 
         $w/o$ multifaceted feedback & 77.40 & 49.18 \\
    \bottomrule
    \end{tabular}
    \label{tab:ablation}
\end{table}
\begin{figure}[t]
    \centering
    % \small
    \includegraphics[width=0.48\textwidth]{Figures/optimizer.pdf} \\
    \caption{Ablation study of optimizer model.}
    \label{fig:optimizer}
\end{figure}
\begin{figure}
    \centering
    % \small
    \includegraphics[width=0.4\textwidth]{Figures/threshod.pdf} \\
    \caption{Ablation of Scoring Threshold ${\beta}$.}
    \label{fig:threshold}
\end{figure}

\subsection{In-Depth Analysis}
\noindent\textbf{Effectiveness of Individual Components.} We further investigate the effectiveness of different modules in our method. We compare our model with the following variants in Table~\ref{tab:ablation}. 

(1) \emph{w/o collaborative reward}. In this variant, we only use execution accuracy $\mathcal{F}_{acc}$ as the reward. This change means {\model} selects optimal chain-of-tool prompts only based on the task performance without considering cooperation between tools action. The results in Table~\ref{tab:ablation} suggest that our collaborative reward mechanism can help {\model} find robust chain-of-tool prompts to improve the generalization of the agent system.

(2) \emph{w/o multifaceted feedback}. Instead of collecting the intermediate execution result of each model, we only feed the final prediction result of the agent system to the optimization model to generate suggestions about prompt refinement. The results shown in Table~\ref{tab:ablation} indicate that multifaceted feedback can motivate {\model} to refine reliable prompts.

\noindent\textbf{Ablation of Optimizer Model.} 
% 说明下summ为啥提示少，llama也不错
We further investigate
the effect of different optimizers used in our model. Specifically, we replace GPT-4 with the open-sourced LLaMA-2~\cite{llama2} to generate insightful suggestions and edit prompts. The results are shown in Figure~\ref{fig:optimizer}. Despite the performance using LLaMA-2 being lower than GPT-4 as expected, we still obtain substantial gain over the initial prompt baseline and surpass previous SOTAs. Such results underscore the robustness of the overall {\model} framework in automatically generating high-quality chain-of-tool prompts, rather than solely relying on the knowledge of optimizer LLM.

\noindent\textbf{Ablation of Scoring Threshold.} 
The highlight of our {\model} is leveraging an optimization model to score the intermediate steps of tool execution by the agent, thereby retrieving tool invocation error from the training data. Thus, we evaluate the influence of different scoring threshold. The results are shown in~\ref{fig:threshold}, which indicates {\model} generally achieves optimal performance with a large scoring threshold ${\beta}$. Additionally, we observe that setting an appropriate scoring threshold for each task is crucial. For instance, tasks like Chart-to-Text, which focus on describing charts, perform well with moderate thresholds. In contrast, tasks such as ChartQA, which involve multi-step tool invocation for complex symbolic reasoning, benefit significantly from higher thresholds.


\input{Tables/prompt_case}
\subsection{Qualitative Analysis}
To provide a direct illustration of how {\model} leverages multifaceted error feedback to refine prompts reliably, we conduct a qualitative analysis
to examine the differences between the prompt optimized by {\model} and other baseline methods. We present a comparison of policy prompt for the ChartQA task, including the normal human-written prompt, the Protegi~\cite{pryzant2023automatic}-optimized prompt, which is edited solely based on prediction error feedback, and the the policy prompt refined by TARO. We further annotate various quality aspects of optimized prompts, highlighting the important perspectives of optimized prompts in advancing prompt engineering, fostering advanced task understanding, and enhancing tool collaboration in LLMs. We summarize the results in Table~\ref{prompt_case}. First, we can observe that, compared to the other two baseline methods, our approach significantly enhances the fine-grained {\ctext[RGB]{230,246,255}{Tool Clarification}} for each tool, helping the LLM establish a clear understanding of the usage conditions for each tool. Second, compared to the \ctext[RGB]{230, 230, 255}{Solution Guidance} aspect of the Protegi-optimized prompt, which emphasizes validating the accuracy of the final result, {\model} provides the LLM with comprehensive insights into tool invocation, such as reminding the model to clarify the expected tool output (e.g., numerical values, labels, etc.), ensure proper integration of data at each step in the sequence, and further adjust the module sequence if the output is incomplete or incorrect. This phenomenon demonstrates that {\model} can identify multifaceted error feedback and seamlessly integrate task-specific and tool-specific knowledge into refined chain-of-tool prompts. Third, from the test performance, the {\model}-optimized chain-of-tool prompts improved the model’s accuracy on ChartQA to 81.20\%, which is 4\% higher than the Protegi-optimized prompt and 7.1\% higher than the human-written prompt. This shows that incorporating sufficient tool invocation instructions in the prompt can significantly enhance the reasoning performance of the model.

\begin{figure}
    \centering
    \small
    \includegraphics[width=0.48\textwidth]{Figures/hqa111.pdf} \\
    \caption{Tool planning error rates on ChartQA and Chart-HQA. Here \textit{incomplete} refers to the insufficient tool action logic to answer the question, while \textit{invalid} means ineffective tool execution results.}
    \label{fig:tool}
\end{figure}
\subsection{Tool Planning Evaluation}
To better illustrate the effectiveness of tool domain knowledge, We follow~\cite{pryzant2023automatic} to use the prediction error feedback to only optimize task prompts while keeping the same parameters as {\model}. We refer to optimized chain-of-tool prompts according to this approach as {\model}-T, which only learn task domain knowledge. We then manually evaluate the tool chains of TARO and TARO-T on 300 randomly selected samples from ChartQA and Chart-HQA respectively. The statistical rates are shown in Fig~\ref{fig:tool}. Here \textit{incomplete} refers to the tool sequence which is not sufficient to solve the question. For example, answering a visual question without invoking the visual perception tool. \textit{invalid} means ineffective tool execution. For example, the agent uses the visual perception tool to query problem-independent visual cues. The results in Figure~\ref{fig:tool} show that {\model} significantly reduces the frequency of incomplete tool chain and the likelihood of ineffective tool actions, thereby improving the accuracy of tool-augmented models on chart-based visual question answering. We also observe that both methods exhibit more serious tool planning problems on Chart-HQA than ChartQA, especially the \textit{invalid} type. This may be attributed to that questions in Chart-HQA need counterfactual reasoning involving multiple chart details, which requires the agent system to not only plan tools, but also know how to use the tool to retrieve multiple relevant chart details.

==> Sections/3_Methodology.tex <==

\section{Methodology}
In this section, we introduce the proposed framework named {\model} in Figure \ref{fig:model} that autonomously optimize chain-of-tool prompts for tool-augmented chart-based visual question answering. In Section \ref{method:problem}, we first formalize the chain-of-tool prompts optimization task. In Section \ref{method:architecture}, we introduce the LLM-based agent system architecture in {\model}. Then, in Section \ref{method:auto}, we present how {\model} leverages multifaceted feedback of the execution process for reliable chain-of-tool prompts refinement. Finally, in Section \ref{method:iterative}, we show how to apply our collaborative reward strategy to search chain-of-tool prompts efficiently.
\subsection{Problem Formulation}
\label{method:problem}
Following a standard setting in prompt optimization \cite{shin2020autoprompt, deng-etal-2022-rlprompt}, we formulate the chain-of-tool prompts optimization problem as a black-box optimization problem guided by LLMs. To be specific, Let $\mathcal{M}$ and $\mathcal{P}_{0}$ represent the set of models and initial natural language chain-of-tool prompts respectively. We use $\mathcal{I}_{\mathcal{P}}$ to represent the LLM-based agent system with the chain-of-tool prompts $\mathcal{P}$, where $\mathcal{I}_{\mathcal{P}} = \{\mathcal{M}, \mathcal{P}\}$. The set of training samples from ChartQA task can be denoted as $\mathcal{D}_{train} = \{q_i, a_i\}^{N}_{i=1}$, where $q_i/a_i$ is the question/answer pair for each sample. Given the question $q_i$ as input, the LLM-based agent system $\mathcal{I}_{\mathcal{P}}$ makes the prediction $\mathcal{M}(q_i, \mathcal{P})$. The goal of chain-of-tool prompts optimization is to find the optimal natural language prompt set $\mathcal{P}^*$
that maximizes the task performance towards a score function $\mathcal{R}$ (e.g., relaxed accuracy), as written with Eq.~\eqref{eq:agent}:
\begin{equation}
\label{eq:agent}
\mathcal{P}^* =  \underset{\mathcal{P}\in {\mathcal{S}}}{\mathop{\arg\max}} \sum_{i=1}^{N} \mathcal{R}(a_i, \mathcal{M}(q_i, \mathcal{P})), 
\end{equation}
where $\mathcal{S}$ denotes the infinitely large search space for agent natural language prompts. Notably, the existing state-of-the-art method DePlot~\cite{liu-etal-2023-deplot} can be formulated as a agent system with raw prompt, denoted as $\mathcal{I}_{\mathcal{P}_{0}} = \{\mathcal{M}, \mathcal{P}_{0}\}$, where $|\mathcal{M}| = 2$.
\subsection{LLM-based Agent System Architecture Design}
\label{method:architecture}
In this section, we present the LLM-based agent system architecture of {\model}. Following the paradigm of "planning then action" in LLM-based autonomous agents ~\cite{wang2023survey}, we design a planning model to organize multiple action models or tools to complete the process of extracting relevant information from the chart and performing symbolic reasoning based on the extracted context. Specifically, our system contains the following five essential models. The initial chain-of-tool prompts are shown in Appendix \ref{app:mutli-agent}.

\noindent\textbf{Policy model.}
This model is primarily responsible for breaking down the original chart question into sub-tasks and planning a set of action models that are executed sequentially to answer the question. 

\noindent\textbf{Data Retrieval model.} This action model extracts data attributes from a given chart image. Inspired by the success of plot-to-text translation in DePlot \cite{liu-etal-2023-deplot}, the data retrieval model translates data information from the chart into easily understandable structured tables from a data-centric view. This structured information further aids large language models in understanding and reasoning about chart content.

\noindent\textbf{Visual Retrieval model.} Beyond querying numerical properties, users often pose questions referring to visual attributes in charts~\cite{chartqa, kim2020answering} (e.g., “What is the value of the rightmost bar?”). The visual retrieval model extracts additional visual knowledge critical to addressing these questions. For example,when querying the rightmost bar, this model identifies its legend label, providing valuable contextual information.

\noindent\textbf{Program model.}
Program-aided methods have demonstrated their ability to enhance the logical and mathematical reasoning capabilities of LLMs~\cite{gupta2023visual, Suris_2023_ICCV}. Since complex chart reasoning often involves arithmetic and logical operations~\cite{chartqa}, the program action model utilizes context from other models to write and execute Python programs via a Python compiler, effectively addressing queries requiring advanced reasoning.

\noindent\textbf{Solution model.}
This model generates a detailed solution to the input query using all the cached information. Employing a chain-of-thought reasoning approach~\cite{wei2023chainofthought}, it ensures coherent and well-structured responses.

\subsection{Reliable Prompts Refinement}
\label{method:auto} 
In order to tackle the reasoning hallucination challenge posed by LLM-based agent system, we propose leveraging the human-like intelligence potential of LLMs to simulate the iterative process through which human users rewrite prompts via trial-and-error, thereby reliably refining structured chain-of-tool prompts. Specifically, we denote chain-of-tool prompts set at the $t$-$th$ iteration as $\mathcal{P}_t$. In each round of prompts refining, there are following two key steps to perform.

\noindent\textbf{Multifaceted Error Feedback Collection.} 
To jointly learn fine-grained task domain knowledge and tool domain knowledge, we focus on identifying prediction errors and tool invocation errors within the LLM-based agent system on training samples. Unlike directly leveraging ground truth labels from downstream tasks to assess prediction errors, evaluating the rationale of the tool execution sequence lacks explicit supervision signals. To address this, inspired by the self-reflection capabilities of LLMs~\cite{shinn2023reflexion}, we employ an additional LLM (e.g., GPT-4) as an optimization model, denoted as $\mathcal{O}$, to evaluate the reasonableness of the tool trajectory. Specifically, as illustrated in Fig~\ref{fig:model}, the optimization model first parses the question and extracts key queries related to the charts. Subsequently, it gathers the intermediate execution results from each model in the current tool action path.
Finally, the optimization model $\mathcal{O}$ assigns a score ranging from 1 to 10 to the tool chain based on a scoring rubric (detailed in Appendix~\ref{}) that was manually designed according to two principles: (1) whether each step faithfully utilizes the results from the preceding tool, and (2) whether the tools accurately query the chart details specified in the question. If the score falls below a predefined threshold ${\beta}$ (a hyperparameter), the tool chain is considered erroneous. During the $t$-th iteration, errors identified in the LLM-based agent system on minibatches of training data are aggregated to form a set of multifaceted error feedback, denoted as $f_t$.

% To jointly learn fine-grained task domain knowledge and tool domain knowledge, we consider recognizing prediction errors and tool invocation errors from the LLM-based agent system on training samples. However, compared to directly using ground truth labels from downstream tasks to assess prediction errors, the rationale of the tool execution sequence lacks direct supervision signals. Therefore, inspired by the success of self-reflection~\cite{shinn2023reflexion} ability of LLMs, We employ an additional LLM (e.g., GPT-4) to serve as an optimization model $\mathcal{O}$, evaluating the reasonableness of the tool trajectory. Specifically, as shown in Fig~\ref{fig:model}, We first let the optimization model parse the question and extract key queries involving the charts. Subsequently, we collect the intermediate execution results of each model in the current tool action path. Finally, the optimization model $\mathcal{O}$ assigns a score from 1 to 10 to the current tool chain based on two principles: whether each step faithfully utilizes the results from the previous tool and whether the tools accurately query the chart details specified in the question. If the score falls below a predefined threshold ${\beta}$, which is a hyper-parameter, the tool chain is deemed erroneous. In the $t$-$th$ iteration, we collect the errors of the LLM-based agent system on minibatches of training data to form a set of multifaceted error feedback, denoted as $f_t$.




% Finally, we determine the tool invocation error based on whether the intermediate execution results respond to the extracted key information. 

% we first  collect the intermediate execution result of each model in the action sequence, then 
%想想怎么设计识别工具调用错误
% Subsequently, we collect the intermediate execution result of each model in the error instance to form a set of multifaceted error feedback, denoted as $f_t$. 

% To accurately locate specific causes of error execution results in LLM-based agent systems, When the multi-agent system $\mathcal{I}_{\mathcal{P}}$ makes errors on the training samples, we collect the intermediate execution result of each model in the error instance to form a set of multifaceted error feedback, denoted as $f_t$. 

\noindent\textbf{Insightful Suggestion Generation.} 
After collecting multifaceted error feedback, we further prompt the optimization model $\mathcal{O}$ to summarize the reasons why current agent system produce errors, extract insightful domain knowledge, and then generate fine-grained suggestions $a_t$ for refining chain-of-tool prompts with Eq.~\eqref{eq:sug}: 
\begin{equation}
\label{eq:sug}
a_t = \mathcal{O}(f_t).
\end{equation}
Subsequently, the optimization model utilizes these generated suggestions to edit the current chain-of-tool prompts $\mathcal{P}t$, producing $\mathcal{K}$ candidate prompts for refinement, as described in Eq.~\eqref{eq:rewrite}:
\begin{equation}
\label{eq:rewrite}
\mathcal{P}_{t+1} = \mathcal{O}(a_t, \mathcal{P}_t).
\end{equation}

\subsection{Efficient Prompts Optimization via Collaborative Reward}
\label{method:iterative}
To address the challenge of searching for optimal chain-of-tool prompts within an infinitely large search space, we introduce a reward mechanism to guide the optimization model $\mathcal{O}$ in efficiently refining chain-of-tool prompts. Most existing prompt optimization approaches rely on task performance (execution accuracy) as the primary reward signal to optimize single prompt~\cite{ape, wang2023promptagent, chen2024improving}. However, in addition to task performance, the cooperation among multiple tools plays a crucial role in determining the overall quality of an LLM-based agent system. To account for this, we propose a collaborative reward mechanism that provides comprehensive feedback to the optimization model. Specifically, for each sample, we define $\mathcal{F}{acc}$ as the execution accuracy of the LLM-based agent system, represented as a binary value (0 or 1). Additionally, the optimization model reflects on the multifaceted error feedback to assess whether each model accurately receives messages from others and fulfills its designated task, calculating the execution coordination $\mathcal{F}{coo}$, also a binary value (0 or 1). The collaborative reward $\mathcal{R}$ for each sample is then calculated as follows:
\begin{equation}
\label{eq:reward}
\mathcal{R} = \mathcal{F}_{acc} \cdot \mathcal{F}_{coo} + \alpha(\mathcal{F}_{coo} - \mathcal{F}_{acc}),
\end{equation}
where $\alpha \in (0, 1)$ is a balance parameter. Further, we combine our collaborative reward mechanism with a regular search algorithm (e.g., beam search) to mitigate the exploration-exploitation trade-off. We leave more advanced search algorithms for future work. The overall training procedure are summarized in Algorithm~\ref{alg:taro}.

\noindent\textbf{Analysis of collaborative reward.} To better understand the proposed collaborative reward mechanism, we provide an analysis of Eq.\ref{eq:reward}. The collaborative reward assigns different values based on the execution state of the LLM-based agent system. Specifically, it provides positive rewards when the tools successfully cooperate, promoting alignment and collaboration among models. Conversely, it penalizes cases where the model "\textit{cheat}" the correct answer without proper cooperation. This approach aligns with the principles of standard reward shaping~\cite{hu2020learning}, ensuring that the optimization process emphasizes both accuracy and coordination within the system.

\begin{algorithm}[t]
\caption{chain-of-tool prompts Optimization with {\model}}
\label{alg:taro}
\begin{algorithmic}[1]
\REQUIRE{$\mathcal{P}_{0}$: initial prompts, $L$: beam width, $T$: iteration number, $\mathcal{K}$: edit count, $\mathcal{R}$: reward function, $\mathcal{D}_{tr}$: train data}\STATE $B_0 \leftarrow \{p_0\}$
\FOR{$i \leftarrow 1$ to $T$}
    \STATE $C \leftarrow \emptyset$
    \FORALL{$p \in B_i$}
        \STATE Sample minibatch $\mathcal{D}_{mini} \subset \mathcal{D}_{tr}$
        \STATE Evaluate prompt $p$ on minibatch $\mathcal{D}_{mini}$ and collect multifaceted error feedback
        \STATE Get insightful suggestion using Equation~\ref{eq:sug}
        \STATE Use the suggestion to edit the current prompt $\mathcal{K}$ times to obtain the prompt candidate set ${P_\mathcal{K}}$ based on Equation~\ref{eq:rewrite}
        \STATE $C \leftarrow C \cup {P_\mathcal{K}}$
    \ENDFOR
    \STATE Select the top $L$ prompt candidates $C_L$ with the highest reward scores from $C$ based on Equation~\ref{eq:reward}
    \STATE $B_{i+1} \leftarrow C_L$
\ENDFOR
\STATE $\hat{p} \leftarrow argmax_{p \in B_r} R(p)$
\RETURN $\hat{p}$
\end{algorithmic}
\end{algorithm}




==> Tables/case.tex <==
\begin{table*}[th!]
% \Large
\caption{The first row shows the split of the relevance of image-text pairs, and the several middle rows indicate representative samples together with their entity-object attention and token-wise similarity in the test set of MNRE datasets, and the bottom five rows in the figure show predicted relation of different approaches on these test samples.
}
\label{tab:re_case}
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{p{9cm}p{9cm}}
\toprule[2pt]
    Factoid QA
    & Hypothetical QA
\\
\midrule[1pt]

\textbf{Question}: Is the average of blue bars greater than the median of all the bars in the East category?  \textbf{Answer}: No
% Infinity War Director Confirms \colorbox{red!30}{Hulk} is NOT Afraid of \colorbox{yellow!30}{Thanos}.
&
% History beckons as \colorbox{red!30}{Trump} - \colorbox{yellow!30}{Kim} summit kicks off in Singapore.
\textbf{Question}: How many people would say "likely" if the value of the slice with color light blue halved and was added to "Very likely"?
\textbf{Answer}: 53
\\
\raisebox{-0.94\totalheight}{
    \includegraphics[width=0.96\linewidth]{figs/re_case_1.png} 
} & 
\raisebox{-0.94\totalheight}{
    \includegraphics[width=0.97\linewidth]{figs/re_case_4.png} 
}
% \\
% \textbf{Gold Relations:} 
%  per/per/peer & per/per/peer
\\
% \midrule[1pt]

% \renewcommand\arraystretch{0.7}
% \begin{tabular}[t]{lll}
%     BERT:  & \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/couple & \xmark\\
%     VisualBERT: & \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/peer & \ding{52}\\
%     MEGA: & \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/peer & \ding{52}\\
%     {Ours}: & \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/peer & \ding{52} \\
%     {Ours}(w/o CAF): & \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/peer & \ding{52} \\
% \end{tabular} &

% \renewcommand\arraystretch{0.7}
% \begin{tabular}[t]{lll}
%      \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/peer & \ding{52} &\\
%     \colorbox{red!30}{per}/\colorbox{yellow!30}{org}/member\_of & \xmark &\\
%     \colorbox{red!30}{per}/\colorbox{yellow!30}{loc}/place\_of\_residence & \xmark &\\
%      \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/peer & \ding{52} \\
%      \colorbox{red!30}{per}/\colorbox{yellow!30}{per}/member\_of & \xmark
% \end{tabular} \\

\bottomrule[2pt]
\end{tabular}
}
\end{table*}



\begin{table*}[tbhp!]
\centering
\small
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\toprule
\raisebox{-0.20\totalheight}{
    \includegraphics[width=0.1\linewidth]{Figures/case_pie.pdf}
}&\multicolumn{5}{c}{\makecell[l]{Q: How many people would say 'likely' \\if the value of the slice with color light blue halved and was added to "Very likely"? \\A:56
}}  \\ 
 \cmidrule(l){2-6}                      
 &Policy&Data\_Retrieval&Visual\_Retrieval &Progam &Output \\
\midrule
\multirow{5}{*}{{\model}-T}
&Data \rightarrow {Program}&\raisebox{-0.20\totalheight}{
    \includegraphics[width=0.1\linewidth]{Figures/case_table.pdf}
} &None&4&5
\\

% \midrule
% \multirow{4}{*}{\model}
% &PROMPTCHART~\cite{promptchart}&81.44&63.20&72.32&-&-&-&-&-&-\\
% &DOMINO~\cite{domino}&\underline{91.80}&\underline{64.10}&\underline{78.00}&-&-&-&-&-&-\\
% &DePlot (GPT3.5)~\cite{liu-etal-2023-deplot}&\underline{91.80}&61.60&76.70&52.80&\underline{59.50}&56.15&\underline{18.30}&\underline{44.50}&\underline{31.40}\\
% &\textbf{{\model}} (GPT3.5) &\textbf{93.20}&\textbf{69.20}&\textbf{81.20} & \textbf{64.90} &\textbf{68.70}&\textbf{66.80}&\textbf{21.20}&\textbf{48.78}& \textbf{34.99}      
\\ 
\bottomrule
\end{tabular}}
\caption{Results on chart-based visual question answering tasks. Comparison with SOTA end-to-end MLLMs and tool-augmented models.}
\label{tab:chart_experiment}
\end{table*}

==> Tables/chart_experiment.tex <==
\begin{table*}[tbhp!]
\centering
% \small
\caption{Results on chart-based visual question answering tasks. Comparison with SOTA end-to-end MLLMs and tool-augmented models.}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{c|l|ccc|ccc|ccc}
\toprule
 \multirow{2}{*}{Type}&\multirow{2}{*}{Models}&\multicolumn{3}{c|}{ChartQA}   & \multicolumn{3}{c|}{ChartCheck} & \multicolumn{3}{c}{Chart-to-text} \\ 
 \cmidrule(l){3-11}                      
 &&Aug.&Human&Avg. &Test1 $F_1$ &Test2 $F_1$&Avg.&Pew&Statista&Avg. \\
\midrule
\multirow{5}{*}{End-to-end}

&Pix2struct~\cite{lee2023pix2struct}&81.60&30.50&56.00  & 44.22 & 45.56&44.89&10.30&38.00&24.15 \\
&MatCha~\cite{liu-etal-2023-matcha}&90.20&38.20 &64.20 &46.40 &48.30&47.35&12.20&39.40&25.80 \\
&Unichart~\cite{masry-etal-2023-unichart} &88.56&43.92&66.24 & 47.90 &44.53 &46.22 &12.48&38.21&25.35 \\
&ChartLlama~\cite{han2023chartllama} &90.36&48.96&69.66 & \underline{56.82}  & 58.42&\underline{57.62}&14.23&40.71&27.47 \\
&ChartVLM-L~\cite{xia2024chartvlm} & 78.12 & 32.91 & 55.52 & 51.75 & 50.08&50.92&16.58 & 41.12&28.85 \\
\midrule
\multirow{4}{*}{Tool-augmented}
&PROMPTCHART~\cite{promptchart}&81.44&63.20&72.32&-&-&-&-&-&-\\
&DOMINO~\cite{domino}&\underline{91.80}&\underline{64.10}&\underline{78.00}&-&-&-&-&-&-\\
&DePlot (GPT3.5)~\cite{liu-etal-2023-deplot}&\underline{91.80}&61.60&76.70&52.80&\underline{59.50}&56.15&\underline{18.30}&\underline{44.50}&\underline{31.40}\\
&\textbf{{\model}} (GPT3.5) &\textbf{93.20}&\textbf{69.20}&\textbf{81.20} & \textbf{64.90} &\textbf{68.70}&\textbf{66.80}&\textbf{21.20}&\textbf{48.78}& \textbf{34.99}      
\\ 
\bottomrule
\end{tabular}}
\label{tab:chart_experiment}
\end{table*}

==> Tables/opt.tex <==
\begin{table}[thbp]
    \centering
    \caption{Ablation study of optimizer model.}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|cccc}
    \toprule
        Optimizer & ChartQA & ChartCheck&Chart-to-text&Chart-HQA  \\ \midrule
        Initial Prompt &74.10 &55.71 &31.15&48.82 \\
        \midrule
         LLaMA-2(13B)&79.20 &62.35  &32.53 &53.46\\
         GPT-4& \textbf{81.20}&\textbf{66.80} & \textbf{34.99} & \textbf{56.89} \\ 
        \bottomrule
    \end{tabular}}
   \label{tab:optimizer}
\end{table}

==> Tables/prompt_case.tex <==
\begin{table*}[t]
% \vspace{-2mm}
\caption{
Policy prompt comparison for the ChartQA task, including normal human prompt, ProTeGi-optimized prompt, and expert-level prompt optimized by {\model}. We highlight different aspects of policy prompt with colors, including \ctext[RGB]{233,252,232}{Task Description}, \ctext[RGB]{230,246,255}{Tool Clarification}, \ctext[RGB]{230, 230, 255}{Solution Guidance}. (Best view with colors). Both baselines primarily focus on task descriptions, while our expert prompt incorporates finer-grained tool instructions and insights that encourage the model to construct rational tool chain, resulting in superior performance. The differences between our method and the baselines are highlighted in \textbf{BOLD TEXT}.
}
\label{prompt_case} 
% \vspace{-1mm}
% \small
\definecolor{Gray}{gray}{0.90}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\centering
\resizebox{0.82\linewidth}{!}{%
\begin{tabular}{@{}lp{10.2cm}c@{}}
\toprule
Approach    & Optimized Policy Prompt & Acc. \\ \midrule
Human       &   \ctext[RGB]{233,252,232}{You need to act as a policy model, that given a question and a modular set, determines the sequence of modules that can be executed sequentially can solve the question}. The modules are defined as follows: Program\_Generator: This module generates a python program to answer question. Data\_Retrieval: This module translate the chart to a table. Visual\_Retrieval: This module retrieves visual information from the chart.            &    74.10  \\\addlinespace
ProTeGi         &    You act as a policy model to solve complex queries by determining the optimal sequence of predefined modules for execution. \ctext[RGB]{233,252,232}{Your task is to analyze a given question, map its components to appropriate modules, and ensure their correct sequence to produce the solution}. The available modules are: Program\_Generator: Generates Python code to compute the final answer. Data\_Retrieval: Converts the chart into structured tables for. Visual\_Retrieval: Extracts visual details from charts. \ctext[RGB]{230, 230, 255}{You can execute modules sequentially and validate the final result for accuracy}. &     77.20 \\\addlinespace
{\model} &  
In selecting the correct modules to answer questions related to a chart, \ctext[RGB]{233,252,232}{your task involves a sophisticated analysis of the question to understand which type of information is being requested. The question may require numerical data interpretation, visual comparison of categories, frequency count analysis, or a combination of different information types}. Here are refined guidelines for selecting the appropriate sequence of modules: 
Choose Data\_Retrieval when extracting numerical data from a chart to present it in a tabular format. \ctext[RGB]{230,246,255}{\textbf{Ensure that the retrieved data is complete and contains no duplication or ambiguity}}. 
Use Visual\_Retrieval \ctext[RGB]{230,246,255}{\textbf{if the question demands insights into categories or other specific visual details not captured by the numerical data alone. This may include identifying colors, patterns, or textual annotations}}. 
Deploy the Program\_Generator module to calculate or compare values \ctext[RGB]{230,246,255}{\textbf{when the answer requires numerical analysis or logical processing grounded in the retrieved data}}. 
When indicating your chosen modules, format them like this: Modules: ["Module Name(s)"]. \ctext[RGB]{230, 230, 255}{It is critical to determine the proper sequence based not only on the literal question but also on the type of information required by the inquiry}. Your module selections must provide a comprehensive solution. \ctext[RGB]{230, 230, 255}{\textbf{Remember to clarify the expected output (numerical values, labels, etc.) and ensure proper integration of data from each step in the sequence. If the output of a module is incomplete or incorrect, adjust the sequence of the modules to refine the results}}. & 81.20
\\ \bottomrule
\end{tabular}
}
\end{table*}
